Robot Coverage Path Planning for General Surfaces Using Quadratic Differentials

Robot Coverage Path planning (i.e., provide full coverage of a given domain by one or multiple robots) is a classical problem in the field of robotics and motion planning. The goal is to provide nearly full coverage while also minimize duplicately visited area. In this paper we focus on the scenario of path planning on general surfaces including planar domains with complex topology, complex terrain or general surface in 3D space. The main idea is to adopt a natural, intrinsic and global parametrization of the surface for robot path planning, namely the holomorphic quadratic differentials. Except for a small number of zero points (singularities), each point on the surface is given a uv-coordinates naturally represented by a complex number. We show that natural, efficient robot paths can be obtained by using such coordinate systems. The method is based on intrinsic geometry and thus can be adapted to general surface exploration in 3D.

==> overview.tex <==
%overview

\section{Overview} 

Here we give a quick overview of this paper. First we compute the holomorphic quadratic differential for the input domain, which provides a global, intrinsic parametrization of the domain by complex coordinates. The theory is presented in Section~\ref{sec:prelim} and the algorithms are presented in Section~\ref{sec:algorithm}. 

Below we give an overview of the steps in our path planning algorithm to help guide the readers through the description. 


\bitem
\item Step 1: we compute the holomorphic quadratic differential for the input domain, which provides a parametrization of the domain by complex coordinates. This step is presented in Section~\ref{ssub:Holomorphic_diff}. 

Holomorphic quadratic differentials inherently induce non-intersecting trajectories on a surface -- by fixing the value of one coordinate we trace out trajectories that are either a loop or end at critical points  -- the singular points that were not given coordinates. 

\item Step 2: we locate the zero points and trace out the critical trajectories that end at zero points. These critical trajectories slice the input domain into $3g-3(3n-2)$ pieces, where $g$ is the genus of the input domain and $n$ is the number of holes. The pieces and their adjacency are represented by a graph $G$ in which the vertices are zero points and each edge represents a cell/piece that connects 

\item Step 3: 

\eitem


==> related_2.tex <==
\section{Related Work}

The coverage path planning problem has been studied extensively and one can refer to nice surveys~\cite{Galceran:2013kg,Choset:2001vf} for past work in this area. 

Most work focus on the scenario of a flat domain with obstacles and use a cell decomposition of the domain into simple shapes.
Popular cell decomposition includes classical trapezoid decomposition\cite{Oksanen:2009gz}, boustrophedon cellular decomposition~\cite{Choset:1998cha,Garcia:2004kd,Jin:2011cl,Xu:2011cl},  Morse decomposition~\cite{Acar:2002fx}, slice decomposition~\cite{Wong:2003fk}, various grid-based algorithms~\cite{Kapanoglu:2012bq,Zelinsky:1993te,Cai:2014un}, etc. Most of these approaches are concerned of producing a small number of cells used in the decomposition, and whether the decomposition can be done in the online setting (when the target domain is unknown and to be discovered).

%spanning tree coverage,\cite{Gabriely:2001gb,Zheng:2005kh}

%sampling based coverage algorithm \cite{Galceran:2012ix}

%neural network based coverage,\cite{Luo:2002fa,Yang:2004gq,Yan:2012dk}

Coverage path planning for surfaces in 3D is less investigated. Atkar \etal~\cite{Atkar01exact} extended the Morse decomposition to non-planar surfaces but did not consider obstacles. 
%P .N. Atkar, H. Choset, A.A. Rizzi, E.U. Acar, Exact cellular decomposition of closed orientable surfaces embedded in r3, in: Proc. ICRA Robotics and Automation IEEE Int. Conf, Vol. 1, 2001, pp. 699–704.
Often heuristic algorithms are adopted in application scenarios~\cite{Cheng08time,Galceran13planning,jin11coverage}. 
%P. Cheng, J. Keller, V. Kumar, Time-optimal uav trajectory planning for 3D urban structure coverage, in: IEEE/RSJ International Conference on, Intelligent Robots and Systems, 2008, IROS 2008, 2008, pp. 2750–2757.
%E. Galceran, M. Carreras, Planning coverage paths on bathymetric maps for in-detail inspection of the ocean floor, in: Proc. International Conference on Robotics and Automation, 2013.
%J. Jin, L. Tang, Coverage path planning on three-dimensional terrain for arable farming, Journal of Field Robotics 28 (3) (2011) 424–440. http://dx.doi.org/10.1002/rob.20388. URL:.

The one most relevant was our earlier work for generating a space filling curve~\cite{ban13topology}. But the focus in~\cite{ban13topology} is to find a curve with progressive density -- that is, we want a path such that the distance from any point to the path to be shrinking progressively when the path gets longer. The same as in a followup work~\cite{li15space}. Although quadratic differentials were also used in~\cite{li15space} but how the path is generated is totally different from here.

%Hert \etal~\cite{} considered coverage of a 3D volume. They first project the domain in 2D and use the 2D planar terrain-covering algorithm

%S. Hert, S. Tiwari, V. Lumelsky, A terrain-covering algorithm for an auv, Autonomous Robots 3 (1996) 91–119.

%Previous works that are most related to ours are \cite{Bhattacharya:2013bj}\cite{Bhattacharya:2014vs}, 
%\textbf{I don't see the relevance to our problem, the above two papers compute voronoi diagram in the geodesic metric. I suggest we remove these references.}

%A related problem is called sweeping path problem\cite{Kim:2003gx}, while given a general surface, ensure that this surface can be `visit' or `swiped' by a robot arm with fixed geometric degree fo freedom.

The coverage path problem is also related to various traveling salesman problem (TSP with neighborhoods~\cite{TSPN}), the lawnmower problem (full cover of a region by a path with minimum length)~\cite{LawnMower}, and the sweeping path problem (full coverage by a robot arm of fixed geometric degree fo freedom)~\cite{Kim:2003gx}. Since these problems are sufficiently different we do not survey the results here. 
%TSPN: E.M. Arkin, R. Hassin, Approximation algorithms for the geometric covering salesman problem, Discrete Applied Mathematics 55 (3) (1994) 197–218.
%LawnMower: E.M. Arkin, S.P. Fekete, J.S. Mitchell, Approximation algorithms for lawn mowing and milling, Computational Geometry 17 (1–2) (2000) 25–50. URL: http://www.sciencedirect.com/science/article/pii/S0925772100000158.
